Characterization of biophysical determinants of spatio-temporal calcium dynamics in astrocytes

Most of the functions performed by astrocytes in brain information processing are related to calcium waves. Experimental studies involving calcium waves present discrepant results, leading to gaps in the full understanding of the functions of these cells. The use of mathematical models help to understand the experimental results, identifying chemical mechanisms involved in calcium waves and the limits of experimental methods. The model is diffusion-based and uses receptors and channels as boundary conditions. The computer program developed was prepared to allow the study of complex geometries, with several astrocytes, each of them with several branches. The code structure allows easy adaptation to various experimental situations in which the model can be compared. The code was deposited in the ModelDB repository, and will be under number 266795 after publication. A sensitivity analysis showed the relative significance of the parameters and identifies the ideal range of values for each one. We showed that several sets of values can lead to the same calcium signaling dynamics. This encourages the questioning of parameters to model calcium signaling in astrocytes that are commonly used in the literature, and it suggests better experimental planning. In the final part of the work, the effects produced by the endoplasmic reticulum when located close to the extremities of the branches were evaluated. We conclude that when they are located close to the region of the glutamatergic stimulus, they favor local calcium dynamics. By contrast, when they are located at points away from the stimulated region, they accelerate the global spread of signaling.

==> repair.60315.Bartie_Pinto_8_biblio.tex <==
%
%
% First comes an example EPS file -- just ignore it and
% proceed on the \documentclass line
% your LaTeX will extract the file if required
%%%\begin{filecontents*}{Fig1.eps}

